Towards Standard Criteria for human evaluation of Chatbots: A Survey

Human evaluation is becoming a necessity to test the performance of Chatbots. However, off-the-shelf settings suffer the severe reliability and replication issues partly because of the extremely high diversity of criteria. It is high time to come up with standard criteria and exact definitions. To this end, we conduct a through investigation of 105 papers involving human evaluation for Chatbots. Deriving from this, we propose five standard criteria along with precise definitions.

==> content/old.tex <==
% \section{introduction}

%  We wanted to provide a comprehensive analysis for dialogue quality and wish it could be used to enhance current practices in dialogue evaluation.
  




 
  


% \section{Dialog quality}
% Linguistic annotation task can not be performed fully automatically. The field of automatic evaluation of dialog system has seen tremendous activity in the past five years, with many successful ，methods being proposed(~\cite{lin2004rouge} ~\cite{tao2018ruber}~\cite{zhang2019bertscore}; Each of them is dedicated to improving agreement with human judgment. However, the open-domain dialog system suffers from a more significant one-to-many problem than other natural language generation tasks(machine translation, text summarization), which results in the requirement of human evaluation.Though human evaluation is widely considered as the gold standard for evaluating the dialogue, and dialogue quality is the centrepiece in the human evaluation process, there  hasn't been a detailed study with dialogue quality; Besides, linguistic evaluation task is prone to the variability in language interpretation and subjective judgment. Hence, it is essential to do a comprehensive analysis of dialogue quality.  
 
% \section{The review of criteria in dialogue evaluation tasks}
 
% Instead of focusing on a large number of the dialogue quality dimension, we limited the selection of criteria to 28 dimensions as the motivation of our
% literature review. We also calculated the criteria occurrence frequency of these papers.[insert the table]

% Here we emphasize on three questions in the dialogue \&criteria review  :
% \begin{itemize}
% \item{ How do the papers choose criteria in their dialogue evaluation?}
% \item{How do the papers define criteria in their dialogue evaluation?}
% \item{Were criteria easy to understand?}
%  \end{itemize}
%  \paragraph{Point 1:  Selection of criteria}

% Linguistic evaluation task is prone to the variability in language interpretation and subjective judgment, particularly question selection and dimension definition(e.g., Acute-eval~\cite{lowe2017towards}, spot the bot~\cite{deriu2020spot} and other papers). From the papers we surveyed, some of them apply more than one criterion. In contrast, a few papers use a direct aspect(e.g., overall quality, appropriateness). 

% We are interested in the details of their choice for criteria.  First, agreement determines what they choose as the dialogue criteria. Lowe et al. (2017)~\cite{lowe2017towards}  find that when they study annotation on different domains, agreement is relatively low among workers for each domain. They finally collect human judgment scores on chitchat dialog using the "appropriateness" metric instead of various criteria.  Second, researchers may want to measure specific dimensions of conversation. For example, a smart conversational agent is expected to provide engaging content during conversations~\cite{roller2020open}, while a common dialogue agent response should satisfy not only topic-similarity but also lexical aspects, informativeness, interestingness, and so on)~\cite{ZimingLi2019DG}. Moreover, From annotators' perspective, As Shikib Mehri et al (2020)~\cite{mehri2020usr} discussed, annotators attribute different weights to the specific features, indicates that human judgment on overall quality may have subjective components.  

% All the evidence shows that if we want to measure the dialogue quality by different criteria comprehensively, we may be at risk of getting lower agreement for some criteria; However,  overall quality measurement is a vague concept that results in diverse understanding among annotators without clear and precise definition.
% \paragraph{Point 2:  Definition of criteria} 

% The definitions or questions they put for dialogue criteria are ambiguous;

% Three level:

% 1. clearly express the meaning they hope to annotate and is close to the concept of the word itself; 

% 2. not much clearly express the meaning they hope to annotate but is close to the concept of the word itself;

% 3.  express the meaning for the criteria ambiguously or misuse the criteria. 


%  \paragraph{Point 3: Other details}

 

  

 

% \subsection{Analytics of dialog quality}
% Our recheck starts from the definition used in  human evaluation process. We conducted a comprehensive analysis for human dialog quality by rechecking 114 papers. According to the meaning used in linguistic\&education\&NLP, we clasify the 28 dimensions into seven groups.
% In education and linguistics domain, we focus on the text properties rather than those of humanness. Fluency is the most frequent criteria in dialogue papers(36/54). However, it is not suitable for explaining the characteristic of dialogue.  According to the dictionary definition, Fluency is defined as "the quality or state of being capable of using a language easily and accurately" [merriam-webster]; Meanwhile, in the education \&linguistic domain, it is defined as " The ability to speak/communicate the information/message with ease, minor mistakes are acceptable."  Primarily, it describes one's verbal ability in a second language. 

% We place emphasis on its application in NLP. Let we see some examples:

% [Fluency definition examples... ]
\subsection{Group 1}
\paragraph{Fluency} 
 
In education and linguistics domain, we focus on the text properties rather than those of humanness. Fluency is the most frequent criteria in dialogue papers(36/54). However, it is not suitable for explaining the characteristic of dialogue.  According to the dictionary definition, Fluency is defined as "the quality or state of being capable of using a language easily and accurately" [merriam-webster]; Meanwhile, in the education \&linguistic domain, it is defined as " The ability to speak/communicate the information/message with ease, minor mistakes are acceptable."  Primarily, it describes one's verbal ability in a second language. 

We place emphasis on its application in NLP. Let we see some examples:

[Fluency definition examples... ]


\paragraph{Grammaticality} 
Grammaticality is the 2nd most used criteria in dialog generation.(8/54) According to the dictionary and linguistics, grammaticality is defined as " The state or quality of conforming to grammar rules",  indicates that if the grammar rules and constraints are followed, then the sentence is judged to be grammatical; Especially in linguistic theory, the grammaticality and the acceptability are two different concepts, a grammatical string is not necessarily meaningful(Grammaticality score will be high if a dialogue system just pieces together some words following grammar rules). Hence, what we really concern about a dialogue response is its acceptability, rather than its grammaticality.



\paragraph{correctness} 

\paragraph{readability} 
\paragraph{Understandable} 
\paragraph{comprehensible}
\paragraph{Our definition}
\begin{itemize}
\item{Fluency: One's speaking ability to express the information with ease, minor mistakes are acceptable}
\item{Grammaticality:  The conformity of a response to grammar rules}
\item{correctness: The conformity of a response to grammar rules}
\item{readability: The quality of the response to be understood easily}
\item{Understandable: The quality of the response being understood}
\item{comprehensible: The capability of being understood}	
\end{itemize}



\subsubsection{Group 2}

\paragraph{consistency}: While current systems are relatively good at staying on topic (Roller et al., 2020)~\cite{roller2020open}, perhaps because they still do not really understand what they are saying they may contradict themselves in subsequent sentences. It is generally assumed that once a speaker select certain objective for the dialogue, it must be maintained. Typically, the objective maybe the persona consistency or the topic consistency. 
\subsubsection{Group 3}
\subsubsection{Group 4}
\subsubsection{Group 5}
 


 
\subsubsection{Association}
We also study the association among different evaluation criteria. Figure \ref{Fig.sankey} is the Sankey Diagram, which indicates the relation between criteria in our summary and criteria used in papers.  
% \begin{landscape}
%     \begin{figure} 
%     \centering  
%     \includegraphics[width=\linewidth]{figure/sankey.png} 
%     \caption{Criteria association}  
%     \label{Fig.sankey}  
%     \end{figure}
% \end{landscape}


\section{Related work}
\label{gen_inst}

Although evaluation work come out one after the other in ACL, EMNLP and other conferences, human evaluation hasn't been taken seriously . 

 


  


